Can Rule-Based Insights Enhance LLMs for Radiology Report Classification? Introducing the RadPrompt Methodology

Developing imaging models capable of detecting pathologies from chest X-rays can be cost and time-prohibitive for large datasets as it requires supervision to attain state-of-the-art performance. Instead, labels extracted from radiology reports may serve as distant supervision since these are routinely generated as part of clinical practice. Despite their widespread use, current rule-based methods for label extraction rely on extensive rule sets that are limited in their robustness to syntactic variability. To alleviate these limitations, we introduce RadPert, a rule-based system that integrates an uncertainty-aware information schema with a streamlined set of rules, enhancing performance. Additionally, we have developed RadPrompt, a multi-turn prompting strategy that leverages RadPert to bolster the zero-shot predictive capabilities of large language models, achieving a statistically significant improvement in weighted average F1 score over GPT-4 Turbo. Most notably, RadPrompt surpasses both its underlying models, showcasing the synergistic potential of LLMs with rule-based models. We have evaluated our methods on two English Corpora: the MIMIC-CXR gold-standard test set and a gold-standard dataset collected from the Cambridge University Hospitals.

==> fig/cardiomegaly_mention.tex <==
\begin{tikzpicture}
    % Define the style for the custom node
    \tikzstyle{splitnode}=[
        rectangle split,
        rectangle split parts=2, 
        rounded corners, 
        draw=black, 
        rectangle split draw splits=false,
        rectangle split horizontal=false,
        minimum height=2cm, 
        minimum width=3cm, 
        align=center
    ]

    % Custom command to draw the blue split in the middle
    \newcommand{\bluesplit}[1]{
        \coordinate (A) at ($(#1.north west)!0.5!(#1.south west) + (0.3, 0)$);
        \coordinate (B) at ($(#1.north east)!0.5!(#1.south east) -(0.3, 0)$);
        \draw[blue] (A) -- (B);
    }

    % Draw nodes
    \node[splitnode] (1) at (0,0) {cardiomegaly \nodepart{two} \textcolor{blue}{Observation}};
    \bluesplit{1} % Draw the blue split for node A

    \node[splitnode] (2) at (0,-1.5) {enlarge.* \nodepart{two} \textcolor{blue}{Observation}};
    \bluesplit{2} % Draw the blue split for node B

    \node[splitnode] (3) at (5,-1.5) {.*heart \nodepart{two} \textcolor{blue}{Anatomy}};
    \bluesplit{3} % Draw the blue split for node B

    \node[splitnode] (4) at (0,-3) {size \nodepart{two} \textcolor{blue}{Anatomy}};
    \bluesplit{4} % Draw the blue split for node B

    \node[splitnode] (5) at (5,-3) {.*heart \nodepart{two} \textcolor{blue}{Anatomy}};
    \bluesplit{5} % Draw the blue split for node B

    \node[splitnode] (6) at (0,-4.5) {size \nodepart{two} \textcolor{blue}{Anatomy}};
    \bluesplit{6} % Draw the blue split for node B

    \node[splitnode] (7) at (5,-4.5) {cardiac \nodepart{two} \textcolor{blue}{Anatomy}};
    \bluesplit{7} % Draw the blue split for node B

    % \node[splitnode] (8) at (10,-4.5) {silhouette \nodepart{two} \textcolor{blue}{Anatomy}};
    % \bluesplit{8} % Draw the blue split for node B


    % Connect nodes with a directed arrow
    \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (2.east) -- (3.west) node[midway, above] {located at};

    \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (4.east) -- (5.west) node[midway, above] {modify};

    \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (6.east) -- (7.west) node[midway, above] {modify};

    % \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (8.west) -- (7.east) node[midway, above] {modify};

    % \node[splitnode] (A) at (0,0) {Top of A \nodepart{two} Bottom of A};
    \node[above=2.2cm of 3.north] {\textbf{Mention Extraction Rules}};
\end{tikzpicture}


==> fig/cardiomegaly_uncneg.tex <==
\begin{tikzpicture}
    % Define the style for the custom node
    \tikzstyle{splitnode}=[
        rectangle split,
        rectangle split parts=2, 
        rounded corners, 
        draw=black, 
        rectangle split draw splits=false,
        rectangle split horizontal=false,
        minimum height=2cm, 
        minimum width=3cm, 
        align=center
    ]

    % Custom command to draw the blue split in the middle
    \newcommand{\bluesplit}[1]{
        \coordinate (A) at ($(#1.north west)!0.5!(#1.south west) + (0.3, 0)$);
        \coordinate (B) at ($(#1.north east)!0.5!(#1.south east) -(0.3, 0)$);
        \draw[blue] (A) -- (B);
    }
    \begin{scope}[local bounding box=topPart]

        \node[splitnode] (un1) at (0,0) {resolved \nodepart{two} \textcolor{blue}{Observation:DP}};
        \bluesplit{un1} % Draw the blue split for node A
        
        \node[splitnode] (1) at (6,0) {cardiomegaly \nodepart{two} \textcolor{blue}{Observation:DP}};
        \bluesplit{1} % Draw the blue split for node A

        \node[splitnode] (un2) at (0,-2.5) {normal \nodepart{two} \textcolor{blue}{Observation:DP}};
        \bluesplit{un2} % Draw the blue split for node A

    
        \node[splitnode] (2) at (6,-2.5) {.*heart \nodepart{two} \textcolor{blue}{Anatomy}};
        \bluesplit{2} % Draw the blue split for node B
    
        \node[splitnode] (3) at (11,-2.5) {size \nodepart{two} \textcolor{blue}{Observation}};
        \bluesplit{3} % Draw the blue split for node B

        % Connect nodes with a directed arrow
        \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (un1.east) -- (1.west) node[midway, above] {modify};
        
        \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (3.west) -- (2.east) node[midway, above] {located at};

        \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (un2.east) -- (2.west) node[midway, above] {modify};

        % Enclose nodes A and B in a transparent, light green node
        \node[fit=(2) (3), label=above:{{Mention Extraction} Rule}, fill=blue!20, fill opacity=0.5, inner sep=0.4cm, rounded corners, draw] {};

        \node[fit=(1), label=above:{{Mention Extraction} Rule}, fill=blue!20, fill opacity=0.5, inner sep=0.4cm, rounded corners, draw] {};


    \end{scope}
    \node[above=0.2cm of topPart.north] {\textbf{Negation Rules}};

    \begin{scope}[local bounding box=bottomPart]

        \node[splitnode] (un4) at (0,-6.2) {stable \nodepart{two} \textcolor{blue}{Observation:DP}};
        \bluesplit{un4} % Draw the blue split for node A

    
        \node[splitnode] (4) at (6,-6.2) {.*heart \nodepart{two} \textcolor{blue}{Anatomy}};
        \bluesplit{4} % Draw the blue split for node B
    
        \node[splitnode] (5) at (11,-6.2) {size \nodepart{two} \textcolor{blue}{Observation}};
        \bluesplit{5} % Draw the blue split for node B
    

        \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (un4.east) -- (4.west) node[midway, above] {modify};

        \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (5.west) -- (4.east) node[midway, above] {modify};
    

        % Enclose nodes A and B in a transparent, light green node
        \node[fit=(4) (5), label=above:{{Mention Extraction} Rule}, fill=blue!20, fill opacity=0.5, inner sep=0.4cm, rounded corners, draw] {};
                
    \end{scope} 
    \node[above=0.2cm of bottomPart.north]{\textbf{Uncertainty Rules}};
\end{tikzpicture}



==> fig/spatial_rules.tex <==
\begin{figure*}
    \centering
    \begin{tikzpicture}
        % Define the style for the custom node
        \tikzstyle{splitnode}=[
            rectangle split,
            rectangle split parts=2, 
            rounded corners, 
            draw=black, 
            rectangle split draw splits=false,
            rectangle split horizontal=false,
            minimum height=2cm, 
            minimum width=3cm, 
            align=center
        ]
    
        % Custom command to draw the blue split in the middle
        \newcommand{\bluesplit}[1]{
            \coordinate (A) at ($(#1.north west)!0.5!(#1.south west) + (0.3, 0)$);
            \coordinate (B) at ($(#1.north east)!0.5!(#1.south east) -(0.3, 0)$);
            \draw[blue] (A) -- (B);
        }

            \node[splitnode] (un1) at (0,0) {low.* \nodepart{two} \textcolor{blue}{Anatomy}};
            \bluesplit{un1} % Draw the blue split for node A
            
            \node[splitnode] (sp1) at (5,0) {lung.* \nodepart{two} \textcolor{blue}{Anatomy}};
            \bluesplit{sp1} % Draw the blue split for node A

            \node[splitnode] (sp2) at (10,0) {lesion.* \nodepart{two} \textcolor{blue}{Observation}};
            \bluesplit{sp2} % Draw the blue split for node A


            \node[splitnode] (un2) at (0,-2.5) {left \nodepart{two} \textcolor{blue}{Anatomy}};
            \bluesplit{un2} % Draw the blue split for node A

        
            \node[splitnode] (2) at (5,-2.5) {pleura.* \nodepart{two} \textcolor{blue}{Anatomy}};
            \bluesplit{2} % Draw the blue split for node B
        
            \node[splitnode] (3) at (10,-2.5) {effusion.* \nodepart{two} \textcolor{blue}{Observation}};
            \bluesplit{3} % Draw the blue split for node B

            % Connect nodes with a directed arrow
            \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (un1.east) -- (sp1.west) node[midway, above] {modify};

            \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (sp2.west) -- (sp1.east) node[midway, above] {located at};
            
            \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (3.west) -- (2.east) node[midway, above] {located at};

            \draw[->, >=stealth', red, shorten <=0.2cm, shorten >=0.2cm] (un2.east) -- (2.west) node[midway, above] {modify};

            % Enclose nodes A and B in a transparent, light green node
            \node[fit=(2) (3), label=above:{{Mention Extraction} Rule}, fill=blue!20, fill opacity=0.5, inner sep=0.4cm, rounded corners, draw] {};

            \node[fit=(sp1) (sp2), label=above:{{Mention Extraction} Rule}, fill=blue!20, fill opacity=0.5, inner sep=0.4cm, rounded corners, draw] {};

    
    \end{tikzpicture}
    \caption{Examples of Radpert spatial rules.}
    \label{fig:spatial-rules}
\end{figure*}


==> tab/radprompt_improve_radpert.tex <==
\begin{table*}
    \centering
        {\small
        \begin{tabular}{lllll}
                             \hline
                             & \multicolumn{4}{c}{\textbf{RadPrompt Improvement of Weighted Average F1 Over RadPert (\%)}}      \\
        \textbf{Pathologies} & \textbf{Gemini 1.5 Pro} & \textbf{Llama 2 70B} & \textbf{Claude 3 Sonnet} & \textbf{GPT 4 Turbo} \\ \hline
        Atelectasis          & 6.2 (0.8, 11.7)         & -0.0 (-1.6, 1.7)     & 3.8 (0.6, 7.5)           & 6.2 (0.7, 11.7)      \\
        Cardiomegaly         & -1.4 (-4.0, 1.2)        & 0.7 (-0.9, 2.4)      & -0.2 (-1.5, 1.0)         & 0.7 (-2.8, 4.5)      \\
        Consolidation        & -7.7 (-16.0, 0.1)       & -22.4 (-29.6, -16.2) & -0.6 (-4.2, 3.2)         & 2.4 (-3.8, 9.1)      \\
        Edema                & -0.9 (-3.9, 2.3)        & 0.5 (-0.8, 1.9)      & 0.1 (-0.8, 1.2)          & 1.3 (-1.7, 4.7)      \\
        Enlarged Card.       & -11.6 (-19.1, -5.1)     & -1.5 (-4.0, 0.7)     & -8.0 (-14.1, -2.4)       & -6.5 (-12.8, -0.8)   \\
        Fracture             & -8.5 (-15.7, -1.2)      & -1.2 (-4.0, 1.2)     & -2.0 (-5.2, 0.0)         & -4.5 (-11.7, 3.3)    \\
        Lung Lesion          & -2.4 (-9.2, 4.9)        & -28.4 (-37.9, -19.4) & 2.1 (-5.3, 11.1)         & -2.9 (-14.0, 9.2)    \\
        Lung Opacity         & -5.0 (-8.0, -2.1)       & -0.4 (-1.9, 1.1)     & -0.4 (-2.7, 1.8)         & -0.2 (-3.1, 2.8)     \\
        Pleural Effusion     & 2.0 (0.0, 4.1)          & -0.7 (-2.1, 0.9)     & 3.2 (1.6, 5.0)           & 2.8 (0.4, 5.4)       \\
        Pleural Other        & -10.0 (-20.3, 1.8)      & -4.0 (-12.5, 0.0)    & 0.0 (0.0, 0.0)           & 13.5 (-3.9, 39.7)    \\
        Pneumonia            & 4.2 (-0.1, 9.4)         & -14.8 (-19.8, -9.7)  & 3.0 (0.5, 6.4)           & 4.4 (-0.4, 9.5)      \\
        Pneumothorax         & -0.6 (-3.1, 2.1)        & -3.0 (-5.0, -1.3)    & 2.7 (0.3, 5.6)           & 3.5 (0.8, 7.1)       \\
        Support Devices      & 2.2 (0.5, 4.0)          & -0.2 (-1.2, 0.5)     & 1.2 (-0.0, 2.5)          & 0.2 (-2.4, 2.8)      \\ \hline
        Macro Average        & -2.2 (-3.8, -0.6)       & -5.5 (-6.9, -4.3)    & 0.5 (-0.4, 1.4)          & 1.4 (-0.5, 3.2)      \\
        Weighted Average     & -0.2 (-1.5, 1.2)        & -3.5 (-4.4, -2.7)    & 1.4 (0.7, 2.1)           & 1.9 (0.7, 3.2)       \\ \hline
        \end{tabular}
            \caption{Improvement of weighted-average F1 scores for RadPrompt over the rule-based RadPert on the MIMIC-CXR gold test set.}
    \label{tab:radprompt_improve_radpert}
\end{table*}
